Simplifying Backscatter Deployment: Full-Duplex LoRa Backscatter

Due to the practical challenges in the deployment of existing half-duplex systems, the promise of ubiquitous backscatter connectivity has eluded us. To address this, we design the first long-range full-duplex LoRa backscatter reader. We leverage existing LoRa chipsets as transceivers and use a microcontroller in combination with inexpensive passive elements including a hybrid coupler, inductors, tunable capacitors, and resistors to achieve 78 dB of self-interference cancellation and build a low-cost, long-range, and small-form-factor Full-Duplex LoRa Backscatter reader. We evaluate our system in various deployments and show that we can successfully communicate with a backscatter tag at distances of up to 300 ft in line of sight, and through obstacles, such as walls and cubicles, in a 4,000 ft$^2$ office area. We reconfigure our reader to conform to the size and power requirements of a smartphone, and demonstrate communication with a contact-lens-form-factor prototype device. Finally, we attach our reader to a drone and demonstrate backscatter sensing for precision agriculture with an instantaneous coverage of 7,850 ft$^2$.

==> Solution.tex <==
\section{Our Solution}
\label{sec:solution}

In this work we introduce a full duplex backscatter design based on a deep, low cost and small form factor SI cancellation scheme. We use a hybrid coupler with a two-stage tuning impedance to achieve the required deep cancellation without any additional feedforward path. The cancellation network solely relies on passive components, which minimizes its cost, power consumption an noise contribution.

The block diagram of our implementation is shown in Fig.\ref{fig:block_diagram}. The continuous wave excitation signal is generated by the synthesizer and is amplified by the power amplifier. The power amplifier output is routed to the antenna through the cancellation network. 
The cancellation network is based on a hybrid coupler and depends on accurate tuning of a balanced impedance to track antenna impedance.
The reflected signal from a backscatter tag is received at the same antenna and pass the cancellation network to flow to the receiver. The cancellation network suppresses the SI signal flowing from the power amplifier toward the RX. 
An on-board micro-controller controls the synthesizer, power amplifier, RX and cancellation network. It uses the channel RSSI reported by the receiver to tune the balance impedance.

Next, we will describe the hybrid coupler principle of operation and then describe the two stage tunable impedance used to achieve the deep required cancellation.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]
    {./Figures/block_diagram2.png}
    \vskip -0.05 in
    \hfill
    \caption{\bf System block diagram.}
    \label{fig:block_diagram}
    \vskip -0.1 in
\end{figure}
 
\subsection{Coupler Principle of Operation}
Couplers are extensively used as power combiners and power splitters in RF and microwave circuits. Couplers are four port devices that divide the input power between output and coupled ports, while keeping the fourth port isolated. We can use this property of the couplers to isolate CS and RX. The carrier signal splits between antenna and coupled ports while the RX port remains isolated. The antenna signal splits between CS and RX ports with the fourth port as the isolated one. 

Couplers are reciprocal elements, which means the coupling factor in both direction is similar. In other words, the portion of the signal at the CS port that flows to ANT port is equal to portion of signal at the ANT port that flows to CS port. Ideally, we like all the signal from CS to flow to antenna, and the incoming signal at the antenna to flow to RX. However, by changing the coupling factor, we can direct more signal from CS port to ANT port(i.e. decrease the transmit insertion loss) at the expense of less incoming signal at the ANT port flow to the RX port. (i.e. increasing receive insertion loss) or vice versa. Since our goal is to maximize the communication range, we need to minimize the sum of transmit and receive insertion losses. A hybrid or 3dB coupler, divides the input power at each port equally between the output and coupled (balanced) ports. It has similar transmit and receive insertion losses of 3dB which minimizes the total loss in communication range.

Two factors limit the practical SI cancellation with a hybrid coupler. The first one is the leakage through the coupler, a typical COTS coupler could provide 25dB isolation between the TX and RX ports \cite{X3C09P1} which is far less than our requirement. The second and more important factor is the antenna reflection. We aim at a low-cost backscatter system with a low-cost antenna, which would typically be characterized with a reflection coefficient about -10dB. Since the reflected signal from the antenna port would divide between the RX and TX ports, the antenna reflection could limit the SI cancellation. 

To achieve deeper cancellation, using a tunable impedance at the coupled port is suggested \cite{Jung2011,Keehr2018,liempd_70_2016}. The flow of the excitation signal between coupler ports is shown in Fig.\ref{fig:blockDiagram}. The carrier signal, (red signal), splits between the antenna and balanced ports. The impedance connected to the balanced port is tuned such that the reflection from this port (green signal) cancels out the leakage through the coupler and reflection from the antenna port (purple signal) at the receiver port to achieve deep cancellation at the RX port (blue signal). 

\subsubsection{Antenna Impedance Variation}
In full duplex systems, environmental variations close to the antenna would affect the antenna impedance and modify the SI to the receiver. This means that objects in close proximity can detune the antenna, i.e. change its reflection coefficient. Since the SI cancellation from the hybrid coupler depends on the tunable impedance tracking of the antenna variation, it is important to characterize the antenna variation.
We design a 1.9 inch by 0.8 inch printed coplanar inverted-F antenna and use it to quantify the antenna variation.  The inverted-F antenna is a common choice for projects of this scale for ease of manufacturing and low cost. In order to measure the environmental sensitivity of the antenna, we connect it to a VNA while subject to environmental variation. We place the antenna upright on a table and tune it to 50 Ohms, then S11 was measured while a hand approached the board from the side, from the end near the radiating element, and from the end away from the radiating element, as well as the antenna being moved to approach the table broadside. It was also measured for a hand making contact with the ground-plane and with the radiating element.  
When keeping at least 1cm away from the board, $\Gamma$ can be shown to be no greater than 0.38. When physically touching the antenna, $\Gamma$ reaches a maximum of 0.65 and when touching the ground-plane $\Gamma$ reaches a maximum of 0.43. By placing the antenna in an enclosure, we can ensure no unwanted contact with the device and assume that any environmental disturbances remain outside of the 1cm threshold.
We conclude from the experiment that our test antenna return loss is less than 0.4 in different test conditions.
%We conclude from the experiment that our tunable impedance must at least cover the impedances with $\gamma$ less than 0.38 to track the antenna impedance variation in the tested scenarios. Since there might be other scenarios that we have not seen in our investigation, we target to cover the circle with $\gamma$ less than 0.5 with the tunable impedance.

\begin{figure}[t]
\includegraphics[width=3.3 in]
{./Figures/antenna_stability_v0.png}
\caption{Antenna impedance variation due to objects in its close vicinity.}
\label{fig:antenna_stability}
\end{figure}

\subsection{Two-Stage Tunable Impedance}
The reflection from the tunable impedance connected to the coupler balanced port must cancel out the sum of the leakage through the coupler to the isolated port and the reflection from the antenna port as shown in the Fig.\ref{fig:blockDiagram}. For a detuned antenna such as the ones measured in previous section, the reflection from the antenna is stronger than the leakage. So, the reflection from the tunable impedance should match the amplitude of the reflection from the antenna.
As we show in section \ref{sec:solution} the antenna return loss might be as high as 0.4 due to objects in its close proximity. We design the tuning network to cover all impedances with $\Gamma$ less than 0.5 to account for the manufacturing mismatches.
%Since there might be other scenarios that we have not seen in our investigation, we target to cover all impedances with $\Gamma$ less than 0.5 with the tunable impedance.

We use a tuning impedance topology with 2 fixed inductors and 4 digitally tunable capacitors \cite{liempd_70_2016} to cover the required impedances. The network is terminated with a resistor that absorbs a portion of the power delivered to balance port, while the rest of power reflects back. The inductors and resistors are not tunable, since the tunable capacitors provides the required flexibility and are less expensive. 

\begin{figure}[!t]
    \centering
    \begin{minipage}{.98\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{Figures/2stage.png}
        \vskip -0.05 in
%        \subcaption{Tag block diagram.}
        \hfill
    \end{minipage}
    \begin{minipage}{.48\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{Figures/can_sim/coverage6.png}
        \vskip -0.05 in
%        \subcaption{Tag block diagram.}
        \hfill
    \end{minipage}
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{Figures/can_sim/coverage10_2nd.png}
        \vskip -0.05 in
%        \subcaption{Tag prototype}
    \end{minipage}
    \caption{\bf Cancellation simulation results. (a)Tunable impedance topology. 
(b)Tunable impedance coverage on smith chart.
(c)Second stage fine tuning}
    \label{fig:tunable_imp}
    \vskip -0.1 in
\end{figure}

The cancellation depth of the hybrid coupler based cancellation network depends on how accurately the reflection from the tunable impedance matches to the SI at the receiver port. To achieve deeper cancellation we need very fine resolution for the tunable impedance. However, the commercial of the shelf digital capacitor have limited resolution determined by their step size.
To solve this issue, we introduce a novel technique to fine tune the reflections from the tunable impedance. This approach allows us to achieve deep cancellation only by tuning the impedance connected to the hybrid coupler and to eliminate the need to vector modulators, digital attenuators or phase shifters from the system, which lowers the system cost.
 
As mentioned before, the commercial off the shelf digital tunable capacitors have limited tuning and the capacitors step size limits the achievable cancellation. The key observation that we have is that the tuning network in terminated with a resistor and the majority of the signal flowing to this port is wasted except a small portion that reflects and cancels out the SI at the RX port. We replace the termination resistor at the end of the tuning network with a resistive signal divider and place a second tunable impedance after that as shown in ~\ref{fig:tunable_imp}. The signal going from the first stage toward the second stage and the reflection coming back from the second stage passes the resistive divider, which effectively lowers the impact of impedance changes in the second stage on the overall reflected signal and increases the tuning resolution.

Each capacitor in the second stage has a much finer impact on the overall network impedance, which makes a deep cancellation possible. The high-level characteristics of the tuning network such as tuning range and cancellation bandwidth is still controlled by the hybrid coupler characteristics and the first stage of the network, with the second stage providing the fine resolution to accurately match the reflection from the balanced port with the leakage and reflection from the antenna port. This coarse and fine tuning approach is similar to the hybrid coupler combined with an analog cancellation feed-forward path, with the second stage effectively provide the same functionality as a feed-forward path at lower cost, lower power and no noise contribution.
The resistive divider must be selected to ensure that the fine tuning network can cover the step of the coarse tuning network to prevent any dead zone in the tuning.

%Simulation results
We have simulated our tunable impedance coverage and resolution using Matlab. We plot the tuning network reflection coefficient at 915MHz in Fig.~\ref{fig:tunable_imp}(b) for step size equal to 6 LSBs for each capacitor in the first stage. The plot only shows 1296 state of the tunable impedance out of more than 1 trillion possible ones, and demonstrate that the tuning network can cover the circle with $\gamma < 0.5$.

We show the fine tuning effect of the second stage in Fig.\ref{fig:tunable_imp}. We select an initial state (black dot) and change each capacitors in the first stage by 1LSB to get the 8 red dots. Without the second stage we couldn't select an impedance between these dots. For each of these 9 states, we plot the tuning network reflection coefficient for step size equal to 10 LSBs for each capacitor in the second stage in blue. The blue cloud shows the fine resolution control that we achieve with the second stage. Furthermore, the plot shows that there is no dead zone in between the first stage steps.
%We set the first stage capacitors to fixed values and plot the tuning network reflection coefficients at 915MHz in Fig.~\ref{fig:tunable_imp}(c) for step size equal to 6 LSBs for each capacitor in the second stage. The black circle is the initial point with the second stage capacitors set to their default values and the eight red circles are eight reflection coefficients with the second stage is set to default values and one of the first stage capacitors change by one LSB. The plot shows that the second stage covers more than 1 step size for each capacitor in the first stage and can be used to fine tune the reflection without any dead zone.

Finally, we simulate the achievable cancellation for 500 random points inside the $\Gamma < 0.4$ circle and plot the cancellation CDF in Fig.~\ref{fig:can_sim}. The 1 percentile achievable cancellation is more than 80dB which satisfies our requirement.

%\begin{figure}[t]
%\includegraphics[width=3 in]{./Figures/fd2-sim.png}
%\caption{Tuning network simulation results. (a)Impedance tuning on smith chart (step size for each capacitor is equal to 5 LSBs.) (b) Achievable cancellation for 10 random antenna impedance. }
%\label{fig:fd2-sim}
%\end{figure} 

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]
    {Figures/can_sim/gnuplot/can_cdf.png}
    \vskip -0.05 in
    \caption{\bf Simulated cancellation for 500 random points with $\Gamma < 0.4$.}
    \label{fig:can_sim}
    \vskip -0.1 in
\end{figure}

\subsection{Excitation Source Selection}
The carrier source phase noise is related to cancellation network bandwidth as shown in equation \ref{eq:CR_phn}. Although the topology used for the tuning network has 2 poles and they can be set to two different frequencies to improve the cancellation bandwidth \cite{liempd_70_2016,Khaledian2018}, this would reduces the cancellation at the center frequency. Furthermore, such system requires a wide-band receiver to provide the feedback on the SI power over the entire bandwidth to tune the capacitors. We need deep cancellation at the excitation frequency in our full duplex backscatter system. Also, the SX1276 maximum bandwidth is 500KHz, which is not sufficient to tune a wideband cancellation network.

We simulated the SI cancellation of the hybrid coupler with our proposed two stage tunable impedance at different frequency offsets with respect to the center frequency. For these simulations, we first tune the capacitors to achieve highest cancellation at the carrier frequency and then sweep the  frequency while keeping the capacitors values fixed. Our simulation results shows that the average SI cancellation at 3MHz offset is 47dB. To compensate for the lower SI cancellation at the offset frequencies, we use ADF4351 which has low -153dBc phase noise sidebands at 3MHz offset and satisfies the requirement \cite{ADF4351}. Although the ADF4351 costs \$7 and is more expensive than a cheap frequency synthesizer, it relaxes the offset cancellation requirement and eliminates the need for wideband cancellation and power detection circuitry which justifies its higher price tag.

\subsection{Tuning}
There are 8 digital capacitors in the design of the tunable impedance arranged in two stages, each with 5 control bits. This means that the tunable impedance has $2^{40}$ or approximately 1 trillion unique states. Obviously, we can not try every possible state or save the impedance corresponding to every state in a look up table. Thus, we need an efficient tuning algorithm that can run on a limited resources MCU to find an state with sufficient cancellation quickly. 
As we show in section \ref{sec:system} we need 78dB cancellation at the excitation frequency and any state with such cancellation would be an acceptable answer to our tuning algorithm. There could be more than one such states and we do not need to find the state with the best possible cancellation.   

We use simulated annealing algorithm to tune the capacitors in each stage separately. Simulated annealing is based on the physical process of heating and then slowly decreasing the temperature of a material to minimize the defects in its structure. At each temperature, we take N steps. In each step, we add a random value bounded by a maximum step size to each capacitor and measure the resulted SI using the SX1276 receiver. We accept the new capacitor values as the system state when the SI decreases, or with a temperature dependent probability when the SI increases. We set predefined cancellation thresholds for each stage and stop the search once the thresholds are met. If the first stages reaches the threshold but the second stage fails to do so, we repeat the tuning for the second stage till it converges or we reach the tuning timeout. 


==> challenges.tex <==
\begin{figure*}[t]
\includegraphics[width=6 in]{./Figures/Fig2.png}
\caption{Full duplex challenges}
\label{fig:fd_challenges}
\end{figure*}

\section{Monostatic Challenges}
\label{sec:challenge}

Monostatic backscatter communication might appear easy to accomplish at first glance. The backscatter tag modulates its data using a subcarrier frequency and the receiver uses frequency filtering to attenuate the transmitter leakage signal and recover the tag reflected signal. This intuition would have been true if we have access to ideal signal generators and ideal filters, but in real world we have to consider the non-idealities of practical circuits. 
Monostatic backscatter devices must transmit the excitation signal and receive the tag reflected signal simultaneously through a shared antenna. The main challenge is that the transmitted signal is much stronger than the reflected signal. For example, if the transmitted output power is 30dBm and the received reflected signal power is -130dBm, the transmitter signal is 10000000000000000 times stronger than the received signal. 
We can not directly connect the transmitter output port and receiver input port to one antenna, since the transmitter output power is much stronger than what the receiver can handle. We use a TX-RX isolation block to isolate the receiver from the transmitter signal, often called Self Interference (SI). Because of the huge power difference between the two signals, we must carefully consider the TX and RX non-idealities and design the TX-RX isolation network to suppress the SI as required to prevent any degradation in recovering the weak reflected signal from the tag.

Here, we consider two main limitation in practical transceivers and explain how these limitation affect our system design.

\subsection{RX Blocker Tolerance} 
In radio design, a blocker is a very strong signal in the vicinity of the desired signal. The receiver should filter out the blocker before demodulating the desired signal. In our monostatic backscatter system, the transmitter provides the RF excitation signal for the tag. However, the transmitter signal also appears as strong self interference at the receiver input and should be filtered out.
Practical filters have limited bandwidth to center frequency ratio, which makes it very difficult and expensive to filter an in-band interference at high frequencies. Although SAW, BAW or cavity filters can be used to build sharp filters at high frequencies, they are expensive and are not electrically tunable. A popular lower cost solution is to first down-convert both the desired signal and interference to baseband frequencies and then filter out the interference as shown in Fig. \ref{fig:fd_challenges}. However, this approach forces the high frequency circuits such as the low noise amplifier to pass the TX leakage signal through them which limits the level of interference a receiver can handle. 
Furthermore, baseband filters have limited stopband attenuation. Even a small portion of the interference signal that passes beyond the filter, might drop the desired channel signal to noise ratio for strong interference. 
The receiver blocker rejection performance abstracts all these effects and specifies the strongest interference the receiver can handle with minimal performance degradation.
The TX-RX isolation must ensure that the TX leakage remains below the receiver blocker tolerance for optimum performance.

\subsection{RX Phase noise}
An ideal oscillator generates a pure sine wave, which means all the signal's power is at a single frequency. Real oscillators have phase modulated noise components, which spreads the oscillator power to adjacent frequencies, resulting in noise sidebands. The phase noise is usually expressed in dBC/Hz which specifies the signal power in a 1Hz bandwidth at an offset frequency, compared to the main tone power.
In the frequency down-conversion process in the receiver, the receiver local oscillator main tone combines with the desired signal to generate the desired baseband signal. At the same time, the transmitter leakage signal combines with the receiver local oscillator phase noise sideband and generates a noise signal at the exact same frequency as the desired baseband signal. This noise signal directly degrade the desired signal SNR.
The transmitter leakage cancellation network must ensure that the transmitter leakage power combined with the receiver local oscillator phase noise stays below the receiver noise floor. Since the receiver noise floor and the in-band phase noise power both scale with the receiver bandwidth, the required transmitter leakage cancellation due to the $RX_{LO}$ phase noise is independent of the receiver bandwidth and primarily depends on the receiver LO characteristics.

\subsection{TX Phase noise} 
Similar to the receiver local oscillator, the transmitter local oscillator has phase noise sidebands. The transmitter phase noise at an offset frequency equal to backscatter tag subcarrier modulation frequency is exactly at the same frequency as the desired backscatter signal. Since the two signals have the same exact frequency, they can not be seperated using filtering.
Thus, the transmitter leakage cancellation network must ensure that the transmitter phase noise at the offset equal to tag subcarrier modulation frequency is attenuated below the receiver noise floor. 

\subsection{Required Transmitter Cancellation} 
Now that we explained the important non-idealities in the practical circuits, we can calculate the required TX-RX isolation. 
The blocker rejection and $RX_{LO}$ phase noise specify the maximum tolerable interference for the receiver. Based on the receiver implementation one could be more stringent compare to the other. The cancellation circuit must suppress the leakage below these levels. So, the required cancellation depth at the TX main tone frequency can be calculated by the difference of the TX output power and the maximum tolerable interference. 
On the other hand, the TX phase noise specifies the required cancellation at the receiver frequency. Since this frequency differs from the TX output frequency by the tag subcarrier modulation frequency, this could be a measure of the required bandwidth of the cancellation circuit. These requirements are shown in Fig.\ref{fig:can_req}.

\begin{figure}[t]
\includegraphics[width=3 in]{./Figures/can_req.png}
\caption{Required Cancellation}
\label{fig:can_req}
\end{figure}

Both phase noise and receiver blocker rejection are a function of the offset frequency and typically improve as the offset frequency increases. Thus, we face several trade-offs in selecting the tag subcarrier modulation frequency. From the tag point of view, increasing the subcarrier modulation frequency increases the power consumption and is undesirable. From the monostatic backscatter base station point of view, increasing the offset frequency relaxes the $RX_{LO}$ phase noise and the blocker requirements which reduces the required depth of the SI cancellation. However, since the offset frequency has increased, the required bandwidth of the cancellation network increases. Based on the selected communication standard and the receiver specifications, one has to consider all these trade-offs  and transmitter specifications to select the optimum tag subcarrier modulation frequency.

\subsection{Case Study: LoRa SX1276 receiver}
In this work, we use commercial SX1276 chipset that implement LoRa standard as the receiver. By referring to the chip datasheet we can find the sensitivity, phase noise and blocking rejection characteristics \cite{S1276}. 
The receiver noise floor for 1Hz bandwidth is $10Log(KT)+RX_{NF} = -170dB$. The $RX_{LO}$ phase noise at 2MHz offset is -128dBC/Hz which means if it combines with a -42dBm interference, the resulted noise signal lies at the receiver noise floor. We consider 6dB margin to make sure the noise signal is below the receiver noise floor. Thus, for a 30dBm TX output signal we need at least 78dB SI cancellation. The datasheet specifies that the receiver blocking performance at 2MHz offset as 94dB for when the receiver sensitivity is -137dBm. Which means the receiver can handle blockers up to -43dBm. We conclude that the RX phase noise has the stringent requirement and is the limiting factor for the SX1276 LoRa receiver, and we need 78dB of SI cancellation at the TX main tone frequency. 

==> comp.tex <==
\subsection{Case for \name}
\label{sec:comparison}
In Table~\ref{table:comp} we provide a summary of \cmt{the} state of the art in {\rev full-duplex} backscatter communication and compare it with our \shortname. Our system achieves 6$\times$ longer range {\rev and 18~dB deeper SI cancellation }compared to the best reported FD backscatter system.
{\rev
We have built our system with the COTS components and commodity radios and avoided bulky RF components such as circulators and phase shifters to minimize the solution cost. Our system uses a hybrid coupler in the cancellation network to minimize the sum of Tx and Rx insertion losses and maximize the range.}
% and out performs most HD systems. Only HD LoRa backscatter system has a longer symmetric range of 237.5~m but the evaluation was based on -143~dBm sensitivity protocol at 45~bps and 2.4~sec packet length~\cite{lorabackscatter}. In our design, we limit receive sensitivity to -134~dBm, to ensure that, packets are shorter than 400~ms, the maximum channel dwell time for frequency hopping systems~\cite{FCC}. Additionally, we use a hybrid-coupler architecture to reduce cost which incurs a loss of 7~dB (see ~\xref{sec:impl}). So, in total our link budget is reduced by 16~dB which translates to 2.5~$\times$ range reduction, close to the 90~m range of our system. We believe that this is a reasonable trade-off given the cost and performance of the \shortname system.

==> table-comp-bs.tex <==
\begin{table*}[!t]
\centering
\vskip -0.1in
\caption{Comparison of State of the Art Backscatter Systems}
\begin{tabular}{|l | c | l | l | p{2 cm} |  p{1.75 cm} |}
 \hline
 \rowcolor{lightgray} Technology & Topology & Transmitter, Receiver & Data rate & Asym. Range & Sym. Range \\ [0.5ex] 
 %\hline 
 %Passive WiFi~\cite{passiveWiFi} & HD & CW, Wi-Fi chipset & 1-11~Mbps & 1~m, 30~m & 7~m \\
 \hline 
 Interscatter~\cite{InterTechnology} & HD & BLE, Wi-Fi chipset & 2-11~Mbps & 1~m, 27~m & N.A. \\
 %\hline 
 %BLE backscatter~\cite{Ensworth2017} & HD & CW, BLE %chipset & 1~Mbps & 1~m, 30~m  & 6.5~m \\
 \hline 
 Free Rider~\cite{freerider} & HD & WiFi, WiFi chipset & 10-60~kbps & 1~m, 45~m & 8~m \\
 \hline 
 LoRea-868~\cite{lorea} & HD & CC2420, CC1310 & 2.9~kbps & 1~m, 3400~m & 75~m \\
 \hline 
 LoRa backscatter~\cite{lorabackscatter} & HD & SX1276, SX1276 & 0.018-37.5~kbps & 1~m, 2800~m & 237.5~m \\
 \hline 
 PLoRa~\cite{plora} & HD & Active LoRa node, USRP & 0.097-6.25~kbps & 0.2~m, 600~m & N.A. \\
 \hline 
 BackFi~\cite{backfi2015} &  FD & WARP SDR, WARP SDR & 1-5~Mbps & N.A. & 7~m \\
 %\hline 
 %FD BLE~\cite{BLE-Monostatic} &  FD & CW, BLE chipset %& 1Mbps & N.A. & 3~m \\
 \hline 
 SDR RFID reader~\cite{sdr_rfid} & FD & SX1257 SDR + FPGA & 40-640~kbps & N.A. & 15~m \\
 \hline 
 PV-Powered RFID tags~\cite{pv-rfid} & FD & Impinj Speedway R400 & 40-640~kbps & N.A. & 15~m \\
 \hline 
 \shortname & FD & ADF4351, SX1276 & 0.36-13.6~kbps & N.A & 90~m \\
 \hline 
\end{tabular}
\label{table:comp_bs}
\vskip -0.25 in
\end{table*}

% \begin{table*}[t!]
% \centering
% \vskip -0.1in
% \caption{Comparison of State of the Art Backscatter Systems}
% \begin{tabular}{|c | c | c | c | p{2 cm} |  p{1.75 cm} |}
%  \hline
%  \rowcolor{lightgray} Technology & Topology & Transmitter, Receiver & Data rate & Asym. Range & Sym. Range \\ [0.5ex] 
%  \hline 
%  Passive WiFi [Kellog et al] & HD & CW, Wi-Fi chipset & 1-11~Mbps & 1~m, 30~m & 7~m \\
%  \hline 
%  Interscatter [Lyer et al] & HD & BLE, Wi-Fi chipset & 2-11~Mbps & 1~m, 27~m & N.A. \\
%  \hline 
%  BLE backscatter [Ensworth et al] & HD & CW, BLE chipset & 1~Mbps & 1~m, 30~m  & 6.5~m \\
%  \hline 
%  Free Rider [Zhang et al] & HD & WiFi, WiFi chipset & 10-60~kbps & 1~m, 45~m & 8~m \\
%  \hline 
%  LoRea-868 [Varshney et al] & HD & CC2420, CC1310 & 2.9~kbps & 1~m, 3400~m & 75~m \\
%  \hline 
%  LoRa backscatter [Talla et al] & HD & SX1276, SX1276 & 0.018-37.5~kbps & 1~m, 2800~m & 237.5~m \\
%  \hline 
%  PLoRa [Peng et al] & HD & Active LoRa node, USRP & 0.097-6.25~kbps & 0.2~m, 600~m & N.A. \\
%  \hline 
%  BackFi [Bharadia et al] &  FD & WARP SDR, WARP SDR & 1-5~Mbps & N.A. & 7~m \\
%  \hline 
%  FD BLE [Ensworth et al] &  FD & CW, BLE chipset & 1Mbps & N.A. & 3~m \\
%  \hline 
%  SDR RFID reader [Keehr] & FD & SX1257 SDR + FPGA & 40-640~kbps & N.A. & 15~m \\
%  \hline 
%  PV-Powered RFID tags [Nithin et al] & FD & Impinj Speedway R400 & 40-640~kbps & N.A. & 15~m \\
%  \hline 
%  \shortname [This Work] & FD & ADF4351, SX1276 & 0.36-13.6Kbps & N.A & 90~m \\
%  \hline 
% \end{tabular}
% \label{table:comp}
% \vskip -0.25 in
% \end{table*}

==> table-comp-fdbs.tex <==
\begin{table*}[t!]
\centering
\vskip -0.1in
\normalsize
\caption{Comparison of State of the Art Full-Duplex Backscatter Systems}
\begin{tabular}{|c | l | c | c | c | c | c | c | }
 \hline
 \rowcolor{lightgray} Technology & \makecell{Transmitter,\\ Receiver} & Carrier & Analog SI Can. Arch. & Can. & Range & Cost & Size\\ [0.5ex] 
 \hline 
 BackFi~\cite{backfi2015} & \makecell{WARP SDR, \\WARP SDR} & \makecell{WiFi \\Packet} & \makecell{Circulator + 16-tap \\analog feedforward} & 60~dB & 7~m & High & 4~$\times$~4~in\\
 \hline 
 FD BLE~\cite{BLE-Monostatic} & \makecell{Agilent N5181A, \\nRF58122} & CW & \makecell{20dB Coupler + \\Active tuning network} & 50~dB & 3~m & Medium & N.A.\\
 \hline 
 SDR RFID reader~\cite{Keehr2018}& \makecell{SX1257 SDR \\+ FPGA} & CW & \makecell{10dB Coupler + Atten.\\ + passive components} & 60~dB & 15~m & Low & 7.4~$\times$~1.3~in\\
 \hline 
\makecell{PV-Powered \\RFID tags}~\cite{pv-rfid} & Speedway R400 & CW & N.A. & N.A. & 15~m & High & 7.5~$\times$~6.9~in\\
 \hline 
 \shortname & \makecell{ADF4351,\\ SX1276} & CW & \makecell{Hybrid Coupler + \\passive components} & 78~dB & 90~m & Low & 1.8~$\times$~3.9~in \\
 \hline 
\end{tabular}
\label{table:comp_fdbs}
\vskip -0.25 in
\end{table*}

% \begin{table*}[t!]
% \centering
% \vskip -0.1in
% \normalsize
% \caption{Comparison of State of the Art Full-Duplex Backscatter Systems}
% \begin{tabular}{|c | c | c | c | c | }
%  \hline
%  \rowcolor{lightgray} Technology & Transmitter, Receiver & Analog SI Cancellation Architecture & Can. & Range \\ [0.5ex] 
%  \hline 
%  BackFi~\cite{backfi2015} & WARP SDR, WARP SDR & Circulator + 16-tap analog feedforward & 60~dB & 7~m \\
%  \hline 
%  FD BLE~\cite{BLE-Monostatic} & Agilent N5181A, nRF58122 & 20dB Coupler + Active tuning network & 50~dB & 3~m \\
%  \hline 
%  SDR RFID reader~\cite{Keehr2018}& SX1257 SDR + FPGA & 10dB Coupler + Atten. + passive comp. & 60~dB & 15~m \\
%  \hline 
%  PV-Powered RFID tags~\cite{pv-rfid} & Impinj Speedway R400 & N.A. & N.A. & 15~m \\
%  \hline 
%  \shortname & ADF4351, SX1276 & Hybrid Coupler + passive components & 78~dB & 90~m \\
%  \hline 
% \end{tabular}
% \label{table:comp}
% \vskip -0.25 in
% \end{table*}


% \begin{table*}[t!]
% \centering
% \vskip -0.1in
% \caption{Comparison of State of the Art Backscatter Systems}
% \begin{tabular}{|c | c | c | c | p{2 cm} |  p{1.75 cm} |}
%  \hline
%  \rowcolor{lightgray} Technology & Transmitter, Receiver & Data rate & Can Arch & Can & Range \\ [0.5ex] 
%  \hline 
%  BackFi~\cite{backfi2015} & WARP SDR, WARP SDR & 1-5~Mbps & Circulator + 16-tap analog feedforward & 60~dB & 7~m \\
%  \hline 
%  FD BLE~\cite{BLE-Monostatic} & CW, BLE chipset & 1Mbps & 21~dB Coupler + Active tuning network & 50~dB & 3~m \\
%  \hline 
%  SDR RFID reader~\cite{sdr_rfid}& SX1257 SDR + FPGA & 40-640~kbps & 10dB coupler & 60~dB & 15~m \\
%  \hline 
%  PV-Powered RFID tags~\cite{pv-rfid} & Impinj Speedway R400 & 40-640~kbps & N.A. & N.A. & 15~m \\
%  \hline 
%  \shortname & ADF4351, SX1276 & 0.36-13.6Kbps & Hybrid Coupler+ passive components & 78~dB & 90~m \\
%  \hline 
% \end{tabular}
% \label{table:comp}
% \vskip -0.25 in
% \end{table*}

==> table-comp-ibfd.tex <==
\begin{table*}[t!]
\centering
\vskip -0.1in
\normalsize
\caption{Comparison of State of the Art Full-Duplex Systems}
\begin{tabular}{|c | c | c | c | c | c | c | c | }
 \hline
 \rowcolor{lightgray}  & Analog SI Can. Arch. & Band & Can. & BW. & Power &  Size\\ [0.5ex] 
 \hline 
 Bharadia et al.~\cite{bharadia_full_2013} & \makecell{Circulator + \\ 16 tap analog FIR filter} & 2.4GHz & 60~dB & 40~MHz & 20~dBm & 4 x 4 in\\
 \hline 
 Duarte et al.~\cite{duarte_design_2014} & \makecell{Multiple antenna + \\ auxiliary can. path} & 2.4GHz & 65~dB & 20~MHz & 8~dBm & N.A.\\
 \hline 
 Chen et al.~\cite{Chen2019} & \makecell{Circulator + 2 tap \\frequency domain equalization} & 900~MHz & 52~dB & 20~MHz & 10~dBm & 0.6 x 1.6 in\\
 \hline 
 Korpi et al.~\cite{korpi_full-duplex_2016}& \makecell{Circulator + 3 complex tap \\analog FIR filter} & 2.4~GHz & 67~dB & 40~MHz & 8~dBm & N.A.\\
 \hline 
Chu et al.~\cite{Chu2018} & \makecell{EBD + Double \\RF adaptive filter} & 1.7~GHz & 70~dB & 40~MHz & 12~dBm & Custum ASIC\\ %\multicolumn{2}{|l|}{Custum ASIC} \\
 \hline 
Van liempd et al.~\cite{liempd_70_2016} & EBD + passive components & 2~GHZ & 65~dB & 64~MHz & 27~dBm & Custum ASIC\\
 \hline 
 \shortname & \makecell{Hybrid Coupler + \\passive components} & 900~MHz & 78~dB & 100KHz & 30dBm & 1.0 x 0.3 in\\
 \hline 
\end{tabular}
\label{table:comp_ibfd}
\vskip -0.25 in
\end{table*}
